The nanoPU: Redesigning the CPU-Network Interface to Minimize RPC Tail Latency

The nanoPU is a new networking-optimized CPU designed to minimize tail latency for RPCs. By bypassing the cache and memory hierarchy, the nanoPU directly places arriving messages into the CPU register file. The wire-to-wire latency through the application is just 65ns, about 13x faster than the current state-of-the-art. The nanoPU moves key functions from software to hardware: reliable network transport, congestion control, core selection, and thread scheduling. It also supports a unique feature to bound the tail latency experienced by high-priority applications. Our prototype nanoPU is based on a modified RISC-V CPU; we evaluate its performance using cycle-accurate simulations of 324 cores on AWS FPGAs, including real applications (MICA and chain replication).

==> packages.tex <==
% Fonts
%\usepackage{lmodern}
% \usepackage{marvosym}
% \usepackage[utf8x]{inputenc}
%\usepackage{fontspec}
%\usepackage{pifont}
\usepackage{color, colortbl, xcolor}
\usepackage[textsize=tiny]{todonotes}
\usepackage{epstopdf}

% Figures
\usepackage{graphicx}
% \usepackage{subcaption}
\usepackage{tikz}

% Formal tables
\usepackage{booktabs}  
\usepackage{array}
\usepackage{multirow}
%\usepackage{arydshln}
%\usepackage{dashrule}
%\usepackage{slashbox}
\usepackage{diagbox}
\usepackage{ctable}

% Math stuff
\usepackage{mathtools}
\usepackage{amsmath}
% \usepackage{siunitx}

% Algorithms
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}

%% Additional packages
\usepackage{anyfontsize}
\usepackage{helvet}
\usepackage{xspace} 
\RequirePackage{ifthen}
\RequirePackage{balance}
\usepackage{listings}
\usepackage{multicol}
\usepackage{lipsum}
\usepackage{mwe}
\usepackage{soul}
\usepackage{outlines}
\usepackage{microtype}
\usepackage[capitalise]{cleveref}
\usepackage{enumitem}
\usepackage{soul}
\usepackage[english]{babel}
\usepackage{amsmath}

% Bibliography
%\usepackage[maxbibnames=99]{biblatex}

%% Code listings
\usepackage{riscv}

%% Quotes
\usepackage{epigraph}

\usepackage{authblk}


==> text/background.tex <==
\section{Background and Motivation}

\subsection{Application Trends}
\textbf{CAUTION:} the following is extracted verbatim from the Nebula paper~\cite{nebula}:

\xxx{Online services are deployed in datacenters to deliver high- quality responses to a plethora of concurrent users, with response times small enough to deliver a highly interactive experience. Responding to each query with such low latency often requires datasets to be replicated across servers, and software to be decomposed into multiple tiers which communicate over the network to synthesize a response. Inter-server communication typically occurs in the form of RPCs: a user query triggers a sequence of RPC fan-outs, forming a tree of sub-queries that spans hundreds or thousands of servers [20]. That fan-out requires strict limits on the tail response latency of each service tier [21], commonly referred to as a Service Level Objective (SLO).}

\xxx{We focus on services generating $\mu$s-scale RPCs, because of their unique challenges and growing presence. While already widespread in the form of in-memory data stores, services with this profile are becoming increasingly omnipresent because of the trend toward microservice software architectures [1]–[3]. Fine-grained RPCs are particularly vulnerable to latency degradation, as otherwise negligible overheads become comparable to the RPC’s actual service time. As the frequency of $\mu$s-scale RPCs in the datacenter increases, so does the importance of handling them efficiently.}

\subsection{Architecture Trends}
Offloading more and more functionality to CPUs on smart NICs is not going to help latency critical applications.

\textbf{CAUTION:} the follow is taken directly from the Nebula paper~\cite{nebula}:
\xxx{As microservices imply a growth in communication-to-computation ratio [1], the first necessary step to handle them efficiently is the use of highly optimized network protocols and operating system components. Recent datacenter networking advancements to address this challenge include user-level network stacks (e.g., DPDK [22]), hardware-assisted solutions (e.g., dataplanes [23], [24], Microsoft Catapult [25]), and even at-scale InfiniBand/RDMA deployments [26], whose hardware-terminated protocol drastically shrinks the overhead of network stack processing. The demand for lower latency motivates even more radical proposals to approach the fundamental lower bound of networking latency—propagation delay—via on-server integration of network fabric controllers. Such designs already exist in both academia (e.g., Scale-Out NUMA~\cite{scale-out-numa}, the FAME-1 RISC-V RocketChip SoC~\cite{firesim}) and industry (e.g., Intel Omni-Path [28], Gen-Z [29]). We expect similar latency-optimized solutions to find their way into datacenters soon, in response to the growing demands and latency-sensitive nature of online services.}

\subsection{Four Problems That Cause Poor Tail Latency}
\begin{enumerate}
    \item \textbf{Network congestion.} Sub-optimal congestion control policies, such as TCP, are in widespread use today, which lead to large queueing delays, packet loss, and head-of-line blocking within the network. Recent proposals, such as NDP and Homa, offer very promising alternatives to enable low latency through the network fabric.
    \item \textbf{Load Balancing of requests to cores.} This has been the topic of much recent research (RSS, Shinjuku, RPCValet, Nebula). Poor load balancing policies lead to some cores that are overwhelmed while others sit idle, exacerbating tail latency issues. Cores dedicated to network IO and request dispatching lead to increased latency and become the throughput bottleneck of the system. Message dispatching must be implemented efficiently in NIC hardware. The Join Bounded Shortest Queue (JBSQ) load balancing policy has been recently shown to be a good option~\cite{nebula}.
    \item \textbf{Scheduling of threads on cores.} Modern operating systems schedule application threads at very coarse granularities (e.g. 4ms for Linux). This prevents the possibility of being able to run multiple latency sensitive threads on a single core, which is a requirement for extreme fine-grained computing where the number of threads will often exceed the physical number of cores available. Even state-of-the-art operating systems, which perform scheduling decisions every 5us (Shinjuku), are too coarse grained when messages are processed in < 1us. One of the instances of this problem is demonstrated by the well known Memcached thread imbalance issue - where a Memcached server is configured with more threads than cores and in turn leads to very poor tail latency.
    \item \textbf{Network interface is a second class citizen of the CPU.} CPU pipelines are designed to be tightly integrated with memory, which is treated as a first class citizen, but network IO is treated more like accessing disk - a second class citizen. All network packets today are DMA’d over PCIe between the NIC and the memory hierarchy (either main memory or the LLC). Then there is traditionally a software networking stack to process these packets and produce messages for the applications. This all means that network messages have to go through many layers of processing before even reaching the application, which is of course not ideal for latency critical RPCs. Furthermore, since modern network interfaces utilize the host memory hierarchy for network IO, this can lead to significant memory bandwidth interference and hence poor tail latency, especially as network data rates continue to increase~\cite{nebula}.
\end{enumerate}

==> text/comparing-rpc-schemes.tex <==
%%\begin{table*}[ht]
%%\begin{minipage}[c]{0.35\linewidth}
%%\centering
\includegraphics[width=0.65\linewidth]{figures/rpc-pipeline.pdf}
\captionof{figure}{Various stages of an end-host RPC pipeline. 
%The network stores RPC packets in caches or memory and notifies the core, running the RPC handler; a transport layer ensures reliable delivery, and orders these packets into messages and forwards them to the application. 
\shahbaz{TODO: draw RPC request lines b/w App and transport. And, packets enter the network from outside.}}
\label{fig:rpc-pipeline}
%%\end{minipage}

%%\hfill
%%\begin{minipage}[c]{0.6\linewidth}
%%\centering
%%\footnotesize
%%\begin{tabular}{c c c c c >{\columncolor{Gray}}c}
%%\toprule
%%& Linux            & RAMCloud~\cite{} &               &                & \\
%%& IX~\cite{}       & Shinjuku~\cite{} & RDMA          &                & \\
%%& ZygOS~\cite{}    & Shenango~\cite{} & FaRM~\cite{}  & DDIO           & \\
%%& RPCValet~\cite{} & eRPC~\cite{}     & FaSST~\cite{} & NeBuLa~\cite{} & {\bf \name{}} \\
%%\midrule
%%\multirow{5}{*}{\bf CPUs} & App. & App. & App. & App. & App. \\
%%& Transport & Transport & -- & Transport & -- \\
%%& Thread Sch. & Thread Sch. & Thread Sch. & Thread Sch. & -- \\
%%& --        & Load Bal. & Load Bal.  & --        & -- \\
%%& Memory    & Memory    & Memory     & L1/L2 Cache   & Reg. File \\
%%\hline
%%{\bf I/O} & Packet & Packet & Message & Packet & Message \\
%%\hline
%%\multirow{4}{*}{\bf NIC} & --        & --        & Transport  & --        & Transport \\
%%& --        & --        & --         & --        & Thread Sch. \\
%%& Load Bal. & --        & --         & Load Bal. & Load Bal. \\
%%& Network   & Network   & Network    & Network   & Network \\
%%\bottomrule
%%\end{tabular}
%%\caption{A comparison between the \name{} and various frameworks for low-latency datacenter RPCs. The \name{} implements all stages of an RPC pipeline in the NIC and forwards messages right into the registers at the heart of a CPU core, running the application. \shahbaz{nebula supports reassembly in NIC.}\shahbaz{TODO: replace CPU and NIC with software or hardware, make this distinction explicit. Also, swap first two columns.}}	
%%\label{tbl:comparison-rpc-schemes}
%%\end{minipage}
%%\end{table*}

